Gauge cooling in complex Langevin for QCD with heavy quarks

We employ a new method, "gauge cooling", to stabilize complex Langevin simulations of QCD with heavy quarks. The results are checked against results obtained with reweigthing; we find agreement within the estimated errors. The method allows us to go to previously unaccessible high densities.

==> PaxHeaders.23629/hdm_gc.tex <==
30 mtime=1353426420.067967628
30 atime=1353426432.857288647
30 ctime=1353426420.067967628

